Mitigating Metric Bias in Minimum Bayes Risk Decoding

While Minimum Bayes Risk (MBR) decoding using metrics such as COMET or MetricX has outperformed traditional decoding methods such as greedy or beam search, it introduces a challenge we refer to as metric bias. As MBR decoding aims to produce translations that score highly according to a specific utility metric, this very process makes it impossible to use the same metric for both decoding and evaluation, as improvements might simply be due to reward hacking rather than reflecting real quality improvements. In this work we find that compared to human ratings, neural metrics not only overestimate the quality of MBR decoding when the same metric is used as the utility metric, but they also overestimate the quality of MBR/QE decoding with other neural utility metrics as well. We also show that the metric bias issue can be mitigated by using an ensemble of utility metrics during MBR decoding: human evaluations show that MBR decoding using an ensemble of utility metrics outperforms a single utility metric.

==> tables/human_eval.tex <==
\begin{tabular}{lccccccc}
& all & en-de & zh-en & \makecell{en-sw} & \makecell{en-ha} & \makecell{en-hi} & \makecell{en-ml} \\
Greedy & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.29 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.35 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.98 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.03 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.02 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} 1.74 \\
Reference & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 1.54† & {\cellcolor[HTML]{F07E7E}} \color[HTML]{F1F1F1} 1.42 & {\cellcolor[HTML]{0E8B0E}} \color[HTML]{F1F1F1} 1.91 & {\cellcolor[HTML]{B80000}} \color[HTML]{F1F1F1} 1.41 & {\cellcolor[HTML]{E60000}} \color[HTML]{F1F1F1} 1.25 & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 1.50‡ & {\cellcolor[HTML]{F17979}} \color[HTML]{F1F1F1} 1.94 \\
MetricX & {\cellcolor[HTML]{F27171}} \color[HTML]{F1F1F1} 1.36 & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} 1.67 & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} 2.43 & {\cellcolor[HTML]{F7BCBC}} \color[HTML]{000000} 1.08 & {\cellcolor[HTML]{F08080}} \color[HTML]{F1F1F1} 1.07 & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} 0.70 & {\cellcolor[HTML]{D1FDD1}} \color[HTML]{000000} 1.70 \\
MetricX-QE & {\cellcolor[HTML]{BD0000}} \color[HTML]{F1F1F1} \bfseries 1.52† & {\cellcolor[HTML]{FB2121}} \color[HTML]{F1F1F1} 1.56 & {\cellcolor[HTML]{F64A4A}} \color[HTML]{F1F1F1} 2.18 & {\cellcolor[HTML]{77E077}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{F9D0D0}} \color[HTML]{000000} 1.04 & {\cellcolor[HTML]{F27373}} \color[HTML]{F1F1F1} 1.09 & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 2.60‡ \\
XCOMET-XXL & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FD1010}} \color[HTML]{F1F1F1} 2.31 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
CometKiwi23-XXL & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{FE0909}} \color[HTML]{F1F1F1} 2.32 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
COMET22 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} 1.98 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
AfriCOMET & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{8EF38E}} \color[HTML]{000000} 0.97 & {\cellcolor[HTML]{F93333}} \color[HTML]{F1F1F1} 1.17 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
AfriCOMET-QE & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 1.44* & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} 1.29 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
IndicCOMET & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{DDFEDD}} \color[HTML]{000000} 0.93 & {\cellcolor[HTML]{FB2222}} \color[HTML]{F1F1F1} \bfseries 2.29† \\
rankAvg:all & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{0E8B0E}} \color[HTML]{F1F1F1} 1.91 & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  & {\cellcolor[HTML]{000000}} \color[HTML]{F1F1F1}  \\
rankAvg:noNC & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 1.05‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} 1.12 & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} 1.87 & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 0.75* & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} 0.85 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.78 & {\cellcolor[HTML]{006B00}} \color[HTML]{F1F1F1} \bfseries 1.31* \\
rankAvg:noNCnoLex & {\cellcolor[HTML]{006F00}} \color[HTML]{F1F1F1} \bfseries 1.08‡ & {\cellcolor[HTML]{006800}} \color[HTML]{F1F1F1} 1.14 & {\cellcolor[HTML]{F8C1C1}} \color[HTML]{000000} 2.03 & {\cellcolor[HTML]{007800}} \color[HTML]{F1F1F1} 0.82 & {\cellcolor[HTML]{53C353}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{006800}} \color[HTML]{F1F1F1} 0.71 & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 1.28* \\
mxQE32mxMBR & {\cellcolor[HTML]{F1FEF1}} \color[HTML]{000000} 1.29 & {\cellcolor[HTML]{FEF8F8}} \color[HTML]{000000} 1.36 & {\cellcolor[HTML]{F6B7B7}} \color[HTML]{000000} 2.04 & {\cellcolor[HTML]{ACFCAC}} \color[HTML]{000000} 0.99 & {\cellcolor[HTML]{96F996}} \color[HTML]{000000} 0.98 & {\cellcolor[HTML]{66D266}} \color[HTML]{000000} 0.86 & {\cellcolor[HTML]{F6B7B7}} \color[HTML]{000000} 1.84 \\
\scriptsize{noncQE32noncnolexMBR} & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} \bfseries 1.13† & {\cellcolor[HTML]{FEF8F8}} \color[HTML]{000000} 1.36 & {\cellcolor[HTML]{C8FDC8}} \color[HTML]{000000} 1.97 & {\cellcolor[HTML]{128F12}} \color[HTML]{F1F1F1} 0.86 & {\cellcolor[HTML]{006F00}} \color[HTML]{F1F1F1} 0.87 & {\cellcolor[HTML]{006500}} \color[HTML]{F1F1F1} \bfseries 0.70* & {\cellcolor[HTML]{007900}} \color[HTML]{F1F1F1} \bfseries 1.39* \\
\end{tabular}

==> tables/metric_correlation_kendalltau_nombr.tex <==
\begin{tabular}{lrrrrrr}
& zh-en & en-de & en-ha & en-sw & en-hi & en-ml \\
\hline
XCOMET-XXL & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.229 & {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 0.110 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 0.114 & {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 0.201 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 0.073 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 0.152 \\
\hline
XCOMET-XL & {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 0.289 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.126 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.123 & {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 0.187 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 0.087 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.179 \\
\hline
MetricX & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 0.218 & {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 0.077 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 0.192 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.087 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} 0.154 \\
\hline
MetricX-QE & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 0.245 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 0.046 & {\cellcolor[HTML]{4CA54C}} \color[HTML]{F1F1F1} 0.093 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.166 & {\cellcolor[HTML]{ADD5AD}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 0.130 \\
\hline
CometKiwi22 & {\cellcolor[HTML]{3A9C3A}} \color[HTML]{F1F1F1} 0.233 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 0.107 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.032 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 0.173 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} 0.087 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.179 \\
\hline
\scriptsize CometKiwi23-XL & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 0.236 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 0.094 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 0.113 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 0.138 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.101 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 0.165 \\
\hline
\scriptsize CometKiwi23-XXL & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} 0.223 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 0.080 & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 0.115 & {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} 0.160 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 0.085 & {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.140 \\
\hline
BLEURT & {\cellcolor[HTML]{349934}} \color[HTML]{F1F1F1} 0.240 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.128 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.098 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 0.173 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.083 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 0.146 \\
\hline
YiSi & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 0.167 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 0.049 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} 0.061 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 0.138 \\
\hline
BLEU & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 0.110 & {\cellcolor[HTML]{B7DAB7}} \color[HTML]{000000} 0.059 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 0.106 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.052 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.083 \\
\hline
chrF & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.040 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 0.083 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 0.115 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 0.067 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 0.129 \\
\hline
chrF++ & {\cellcolor[HTML]{DFEDDF}} \color[HTML]{000000} 0.067 & {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 0.045 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 0.084 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 0.118 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 0.064 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 0.123 \\
\hline
TER & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 0.120 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 0.061 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 0.084 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.077 & {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 0.087 \\
\hline
\vtop{\hbox{\strut MetricX}\hbox{\strut +MetricX-QE}} & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.246 & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 0.055 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 0.084 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 0.196 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 0.088 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 0.155 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}} & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 0.277 & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.121 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 0.210 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 0.088 & {\cellcolor[HTML]{0F870F}} \color[HTML]{F1F1F1} 0.186 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}\hbox{\strut +COMET22}} & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.293 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.127 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 0.116 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.213 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 0.090 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.193 \\
\end{tabular}

==> tables/metric_correlation_pearson_nombr.tex <==
\begin{tabular}{lrrrrrr}
& zh-en & en-de & en-ha & en-sw & en-hi & en-ml \\
\hline
XCOMET-XXL & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 0.245 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 0.084 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 0.146 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 0.139 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 0.202 \\
\hline
XCOMET-XL & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.428 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.126 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.154 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 0.160 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.141 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 0.208 \\
\hline
MetricX & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.383 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 0.105 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 0.077 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 0.146 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 0.100 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.216 \\
\hline
MetricX-QE & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 0.401 & {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} 0.120 & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 0.115 & {\cellcolor[HTML]{52A852}} \color[HTML]{F1F1F1} 0.132 & {\cellcolor[HTML]{E8F2E8}} \color[HTML]{000000} 0.074 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 0.170 \\
\hline
CometKiwi22 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 0.257 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.148 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.050 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 0.156 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 0.116 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.235 \\
\hline
\scriptsize CometKiwi23-XL & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 0.246 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} 0.092 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 0.098 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.118 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 0.202 \\
\hline
\scriptsize CometKiwi23-XXL & {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 0.205 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 0.088 & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} 0.116 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 0.121 & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 0.128 & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 0.208 \\
\hline
BLEURT & {\cellcolor[HTML]{68B368}} \color[HTML]{F1F1F1} 0.275 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.152 & {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 0.134 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} 0.143 & {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.115 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 0.205 \\
\hline
YiSi & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 0.221 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 0.088 & {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 0.105 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 0.100 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 0.092 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 0.187 \\
\hline
BLEU & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 0.163 & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 0.095 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.073 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.091 \\
\hline
chrF & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.055 & {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.106 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.106 & {\cellcolor[HTML]{C0DEC0}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 0.164 \\
\hline
chrF++ & {\cellcolor[HTML]{E2EFE2}} \color[HTML]{000000} 0.098 & {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 0.058 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 0.108 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 0.157 \\
\hline
TER & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 0.145 & {\cellcolor[HTML]{C4E0C4}} \color[HTML]{000000} 0.071 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 0.104 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.061 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 0.105 & {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} 0.118 \\
\hline
\vtop{\hbox{\strut MetricX}\hbox{\strut +MetricX-QE}} & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.424 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} 0.101 & {\cellcolor[HTML]{259225}} \color[HTML]{F1F1F1} 0.152 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 0.101 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.229 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}} & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 0.396 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 0.110 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.159 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} 0.161 & {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 0.144 & {\cellcolor[HTML]{0C860C}} \color[HTML]{F1F1F1} 0.228 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}\hbox{\strut +COMET22}} & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 0.397 & {\cellcolor[HTML]{289328}} \color[HTML]{F1F1F1} 0.136 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} 0.150 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.169 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.144 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.235 \\
\end{tabular}

==> tables/metric_correlation_spearman.tex <==
\begin{tabular}{lrrrrrr}
lang & zh-en & en-de & en-ha & en-sw & en-hi & en-ml \\
\hline
metric &  &  &  &  &  &  \\
\hline
XCOMET-XXL & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 0.372 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} 0.141 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 0.147 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 0.261 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 0.197 \\
\hline
\scriptsize XCOMET-XXL:mbr & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 0.373 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.145 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 0.160 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 0.274 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} 0.121 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.199 \\
\hline
XCOMET-XL & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 0.451 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 0.162 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.159 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 0.243 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.233 \\
\hline
\scriptsize XCOMET-XL:mbr & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.453 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 0.172 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.176 & {\cellcolor[HTML]{219021}} \color[HTML]{F1F1F1} 0.260 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 0.120 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 0.219 \\
\hline
MetricX & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 0.346 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 0.100 & {\cellcolor[HTML]{319831}} \color[HTML]{F1F1F1} 0.248 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 0.197 \\
\hline
MetricX:mbr & {\cellcolor[HTML]{299429}} \color[HTML]{F1F1F1} 0.397 & {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} 0.117 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 0.144 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 0.272 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.125 & {\cellcolor[HTML]{5EAE5E}} \color[HTML]{F1F1F1} 0.194 \\
\hline
MetricX-QE & {\cellcolor[HTML]{2A952A}} \color[HTML]{F1F1F1} 0.395 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 0.119 & {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.213 & {\cellcolor[HTML]{D3E7D3}} \color[HTML]{000000} 0.074 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 0.146 \\
\hline
\scriptsize CometKiwi23-XXL & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.355 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 0.104 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 0.149 & {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} 0.207 & {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 0.182 \\
\hline
\scriptsize CometKiwi23-XL & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 0.382 & {\cellcolor[HTML]{67B267}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 0.145 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 0.180 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 0.129 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 0.214 \\
\hline
CometKiwi22 & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 0.372 & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 0.139 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.042 & {\cellcolor[HTML]{52A852}} \color[HTML]{F1F1F1} 0.224 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 0.112 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 0.232 \\
\hline
COMET22 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} 0.370 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 0.131 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 0.081 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 0.231 & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} 0.099 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 0.217 \\
\hline
COMET22:mbr & {\cellcolor[HTML]{299429}} \color[HTML]{F1F1F1} 0.397 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.163 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 0.086 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.236 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.113 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 0.208 \\
\hline
BLEURT & {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 0.378 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 0.165 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 0.126 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.223 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 0.106 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 0.186 \\
\hline
BLEURT:mbr & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 0.375 & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 0.174 & {\cellcolor[HTML]{289328}} \color[HTML]{F1F1F1} 0.154 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} 0.242 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.139 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 0.171 \\
\hline
YiSi & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} 0.247 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 0.064 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{CAE3CA}} \color[HTML]{000000} 0.136 & {\cellcolor[HTML]{C4E0C4}} \color[HTML]{000000} 0.078 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 0.180 \\
\hline
YiSi:mbr & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 0.255 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 0.089 & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 0.156 & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 0.084 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} 0.200 \\
\hline
chrF & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.052 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 0.108 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 0.149 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.167 \\
\hline
chrF:mbr & {\cellcolor[HTML]{C4E0C4}} \color[HTML]{000000} 0.127 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 0.065 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.127 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 0.176 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 0.189 \\
\hline
chrF++ & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 0.079 & {\cellcolor[HTML]{DEEDDE}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 0.108 & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 0.154 & {\cellcolor[HTML]{B7DAB7}} \color[HTML]{000000} 0.082 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 0.159 \\
\hline
chrF++:mbr & {\cellcolor[HTML]{BBDCBB}} \color[HTML]{000000} 0.145 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 0.068 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 0.126 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 0.176 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 0.074 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.183 \\
\hline
sentBLEU & {\cellcolor[HTML]{BDDCBD}} \color[HTML]{000000} 0.141 & {\cellcolor[HTML]{BCDCBC}} \color[HTML]{000000} 0.078 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{C8E2C8}} \color[HTML]{000000} 0.138 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.108 \\
\hline
sentBLEU:mbr & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 0.217 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 0.076 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 0.106 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 0.158 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 0.075 & {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} 0.134 \\
\hline
TER & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 0.178 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 0.080 & {\cellcolor[HTML]{76BA76}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.112 & {\cellcolor[HTML]{81BF81}} \color[HTML]{000000} 0.099 & {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 0.111 \\
\hline
TER:mbr & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 0.158 & {\cellcolor[HTML]{B9DBB9}} \color[HTML]{000000} 0.079 & {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 0.114 & {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 0.127 & {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 0.151 \\
\hline
\vtop{\hbox{\strut MetricX}\hbox{\strut +MetricX-QE}}  & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.390 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} 0.110 & {\cellcolor[HTML]{2A952A}} \color[HTML]{F1F1F1} 0.253 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.198 \\
\hline
\vtop{\hbox{\strut MetricX}\hbox{\strut +MetricX-QE}} & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 0.415 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 0.091 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} 0.139 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 0.263 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 0.196 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}} & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 0.437 & {\cellcolor[HTML]{259225}} \color[HTML]{F1F1F1} 0.159 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 0.156 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 0.272 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.113 & {\cellcolor[HTML]{0F870F}} \color[HTML]{F1F1F1} 0.242 \\
\hline
\vtop{\hbox{\strut \scriptsize XCOMET-XXL:mbr}\hbox{\strut \scriptsize +XCOMET-XL:mbr}} & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 0.437 & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 0.169 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.175 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.280 & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 0.125 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 0.230 \\
\hline
\vtop{\hbox{\strut XCOMET-XXL}\hbox{\strut +XCOMET-XL}\hbox{\strut +COMET22}} & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.465 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 0.164 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.150 & {\cellcolor[HTML]{0C860C}} \color[HTML]{F1F1F1} 0.275 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 0.116 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.252 \\
\hline
\vtop{\hbox{\strut \scriptsize XCOMET-XXL:mbr}\hbox{\strut \scriptsize +XCOMET-XL:mbr}\hbox{\strut +COMET22:mbr}} & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.469 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.179 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 0.167 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.284 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 0.128 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 0.239 \\
\hline
\end{tabular}

==> tables/metric_correlation_spearman_nombr.tex <==
\begin{tabular}{lrrrrrr}
lang & zh-en & en-de & en-ha & en-sw & en-hi & en-ml \\
metric &  &  &  &  &  &  \\
XCOMET-XXL & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.306 & {\cellcolor[HTML]{319831}} \color[HTML]{F1F1F1} 0.141 & {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 0.147 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 0.261 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 0.197 \\
XCOMET-XL & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 0.389 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 0.162 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.159 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 0.243 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 0.233 \\
MetricX & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 0.297 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 0.085 & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 0.100 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 0.248 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 0.197 \\
MetricX-QE & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 0.333 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} 0.119 & {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 0.213 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 0.074 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 0.146 \\
CometKiwi22 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 0.315 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 0.139 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.042 & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 0.224 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.112 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 0.232 \\
CometKiwi23-XL & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 0.319 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.124 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 0.145 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 0.180 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.129 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 0.214 \\
CometKiwi23-XXL & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 0.298 & {\cellcolor[HTML]{7EBE7E}} \color[HTML]{000000} 0.104 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 0.149 & {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} 0.207 & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 0.182 \\
BLEURT & {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 0.324 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.165 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.126 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 0.223 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.106 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 0.186 \\
YiSi & {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} 0.230 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 0.064 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} 0.136 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 0.078 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 0.180 \\
BLEU & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 0.150 & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 0.078 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 0.094 & {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 0.138 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.066 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.108 \\
chrF & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.073 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.052 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 0.108 & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 0.149 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 0.087 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.167 \\
chrF++ & {\cellcolor[HTML]{DEEDDE}} \color[HTML]{000000} 0.091 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 0.108 & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 0.154 & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 0.082 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 0.159 \\
TER & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 0.162 & {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 0.080 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 0.109 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.112 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.099 & {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 0.111 \\
MetricX+MetricX-QE & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.334 & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 0.072 & {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 0.110 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 0.253 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} 0.111 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.198 \\
XCOMET-XXL+XCOMET-XL & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 0.373 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 0.159 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.156 & {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 0.272 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 0.113 & {\cellcolor[HTML]{0F870F}} \color[HTML]{F1F1F1} 0.242 \\
XCOMET-XXL+XCOMET-XL+COMET22 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.396 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 0.164 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 0.150 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.275 & {\cellcolor[HTML]{319831}} \color[HTML]{F1F1F1} 0.116 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.252 \\
\end{tabular}


==> tables/multistep/multistep_all_dev.tex <==
\setlength\tabcolsep{2 pt}
\begin{small}

\begin{tabular}{lrrrrrrrrrrrrrr}
\hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \lrot{\textbf{Evaluated Metric}} & \lrot{XCOMET-XXL} & \lrot{XCOMET-XL} & \lrot{COMET22} & \lrot{MetricX} & \lrot{MetricX-QE} & \lrot{CometKiwi22} & \lrot{CometKiwi23-XL} & \lrot{CometKiwi23-XXL} & \lrot{BLEURT} & \lrot{YiSi} & \lrot{sentBLEU} & \lrot{chrF} & \lrot{chrF++} & \lrot{TER} \\
\textbf{Decoding Method} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
allQE(64)allMBR & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 87.8 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 0.987 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 0.637 & {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} 72.3 & {\cellcolor[HTML]{A0CEA0}} \color[HTML]{000000} 82.3 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 24.1 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 55.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 52.6 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 64.6 \\
allQE(32)allMBR & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 88.0 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 0.956 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 0.600 & {\cellcolor[HTML]{52A852}} \color[HTML]{F1F1F1} 79.7 & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 72.8 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 82.9 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{0E870E}} \color[HTML]{F1F1F1} 23.6 & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 55.4 & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 52.2 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 65.5 \\
allQE(16)allMBR & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{67B267}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 0.942 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 0.568 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} 73.2 & {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{2A952A}} \color[HTML]{F1F1F1} 79.8 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 23.0 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 54.9 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 51.7 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 66.4 \\
allQE(8)allMBR & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 0.937 & {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 0.539 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 80.2 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 73.5 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 83.2 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} 22.1 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 54.2 & {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 51.0 & {\cellcolor[HTML]{ADD5AD}} \color[HTML]{000000} {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 67.7 \\
allQE(4)allMBR & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 0.942 & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 0.515 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 80.4 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 73.8 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} 84.2 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} 79.2 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 21.2 & {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} 53.3 & {\cellcolor[HTML]{52A852}} \color[HTML]{F1F1F1} 50.1 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} 69.5 \\
allQE(64)nolexMBR & {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 88.5 & {\cellcolor[HTML]{349934}} \color[HTML]{F1F1F1} 84.2 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.890 & {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.576 & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 80.5 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 22.7 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 54.7 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 51.5 & {\cellcolor[HTML]{BCDCBC}} \color[HTML]{000000} {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 67.0 \\
allQE(32)nolexMBR & {\cellcolor[HTML]{67B267}} \color[HTML]{F1F1F1} 88.6 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 0.873 & {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} 0.548 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 79.8 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 73.0 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 83.2 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 80.3 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 83.3 & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 22.4 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 54.4 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 51.2 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 67.5 \\
allQE(16)nolexMBR & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 88.6 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} 0.878 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 0.531 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 73.3 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 80.1 & {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 83.1 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} 21.9 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} 54.0 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 50.8 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 68.3 \\
allQE(8)nolexMBR & {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} 88.5 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{7EBE7E}} \color[HTML]{000000} {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 0.879 & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} 0.512 & {\cellcolor[HTML]{188C18}} \color[HTML]{F1F1F1} 80.2 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 73.6 & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 84.0 & {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 79.8 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 82.9 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 21.4 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 53.6 & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 50.3 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 69.1 \\
allQE(4)nolexMBR & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 88.4 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 84.1 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 0.897 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 0.500 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 80.5 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 73.9 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{45A245}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 82.6 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 20.6 & {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 52.8 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 49.5 & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} 70.4 \\
topQE(64)topMBR & {\cellcolor[HTML]{319831}} \color[HTML]{F1F1F1} 89.5 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 85.1 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 86.0 & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} 0.760 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.496 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 79.3 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 73.0 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 83.2 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 79.1 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{9ACB9A}} \color[HTML]{000000} 19.4 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 51.5 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 72.1 \\
topQE(32)topMBR & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 89.4 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 85.0 & {\cellcolor[HTML]{67B267}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 0.778 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 0.484 & {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{3A9C3A}} \color[HTML]{F1F1F1} 73.3 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 79.0 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 51.6 & {\cellcolor[HTML]{8CC58C}} \color[HTML]{000000} 48.3 & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 71.9 \\
topQE(16)topMBR & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 89.2 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} 0.794 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.475 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 73.7 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 84.1 & {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 79.0 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 19.7 & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} 51.8 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 48.5 & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 71.7 \\
topQE(8)topMBR & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 89.1 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 84.6 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.818 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} 0.460 & {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 74.0 & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} 78.9 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 51.7 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 48.4 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 71.9 \\
topQE(4)topMBR & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 88.8 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 86.0 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.847 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 0.446 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 74.2 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 19.4 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 51.4 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 48.1 & {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 72.4 \\
noncQE(64)noncnolexMBR & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 87.2 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} {\cellcolor[HTML]{69B369}} \color[HTML]{F1F1F1} 0.870 & {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} 0.549 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 71.8 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 80.4 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 22.6 & {\cellcolor[HTML]{259225}} \color[HTML]{F1F1F1} 54.6 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 51.4 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 67.1 \\
noncQE(32)noncnolexMBR & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 87.3 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 82.9 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 0.826 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} {\cellcolor[HTML]{5CAD5C}} \color[HTML]{F1F1F1} 0.488 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 71.8 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 80.1 & {\cellcolor[HTML]{359A35}} \color[HTML]{F1F1F1} 83.1 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 21.7 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 53.8 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 50.6 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 68.4 \\
noncQE(16)noncnolexMBR & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 87.3 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{349934}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{9ACB9A}} \color[HTML]{000000} {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 0.804 & {\cellcolor[HTML]{A9D3A9}} \color[HTML]{000000} {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} 0.437 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 71.7 & {\cellcolor[HTML]{B9DBB9}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 82.7 & {\cellcolor[HTML]{70B770}} \color[HTML]{F1F1F1} 20.6 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 52.8 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 49.5 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 70.1 \\
noncQE(8)noncnolexMBR & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} 87.1 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 82.3 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 86.2 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} 0.802 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 0.397 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 79.0 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 19.5 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 51.6 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 48.3 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 71.8 \\
noncQE(4)noncnolexMBR & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} 0.813 & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 0.363 & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 71.2 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 81.1 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{C1DFC1}} \color[HTML]{000000} 18.2 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 50.3 & {\cellcolor[HTML]{B9DBB9}} \color[HTML]{000000} 46.9 & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} 74.1 \\
noncQE(64)noncMBR & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 82.5 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 0.969 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 0.601 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 79.0 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 71.4 & {\cellcolor[HTML]{CBE4CB}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{289328}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 24.0 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 55.6 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 52.4 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 64.7 \\
noncQE(32)noncMBR & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 87.0 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} 82.5 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 86.5 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} 0.911 & {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} 0.523 & {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 79.0 & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 22.9 & {\cellcolor[HTML]{219021}} \color[HTML]{F1F1F1} 54.7 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 51.5 & {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 66.1 \\
noncQE(16)noncMBR & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 87.0 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 86.3 & {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} 0.876 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} 0.460 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 79.1 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 83.0 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 21.7 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 53.6 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 50.4 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} 68.0 \\
noncQE(8)noncMBR & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{70B770}} \color[HTML]{F1F1F1} 86.0 & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 0.860 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} {\cellcolor[HTML]{349A34}} \color[HTML]{F1F1F1} 0.412 & {\cellcolor[HTML]{ADD5AD}} \color[HTML]{000000} 78.8 & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} 71.3 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{81BF81}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 82.4 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 20.3 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 52.3 & {\cellcolor[HTML]{74B974}} \color[HTML]{F1F1F1} 49.0 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 70.3 \\
noncQE(4)noncMBR & {\cellcolor[HTML]{E2EFE2}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{D3E7D3}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 0.862 & {\cellcolor[HTML]{CBE4CB}} \color[HTML]{000000} {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 0.372 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 71.0 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 77.8 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 18.7 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 50.7 & {\cellcolor[HTML]{A9D3A9}} \color[HTML]{000000} 47.4 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 73.1 \\
mxQE(64)xcMBR & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 89.9 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{CCE4CC}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 0.981 & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.528 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} 71.1 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{CAE3CA}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 17.6 & {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 49.3 & {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 46.0 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} 74.5 \\
mxQE(32)xcMBR & {\cellcolor[HTML]{289428}} \color[HTML]{F1F1F1} 89.6 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 85.3 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 0.924 & {\cellcolor[HTML]{A0CEA0}} \color[HTML]{000000} {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 0.454 & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 71.1 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{C8E2C8}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 17.7 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 49.4 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 46.1 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 74.4 \\
mxQE(16)xcMBR & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 89.3 & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{7EBE7E}} \color[HTML]{000000} {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 0.880 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 0.397 & {\cellcolor[HTML]{C0DEC0}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 71.2 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 17.6 & {\cellcolor[HTML]{D7E9D7}} \color[HTML]{000000} 49.3 & {\cellcolor[HTML]{D7E9D7}} \color[HTML]{000000} 46.0 & {\cellcolor[HTML]{259225}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 74.4 \\
mxQE(8)xcMBR & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 88.8 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{D7E9D7}} \color[HTML]{000000} 85.1 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 0.851 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 0.354 & {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 71.0 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 81.5 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 77.2 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 81.1 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 17.4 & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 49.0 & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 45.7 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 74.8 \\
mxQE(4)xcMBR & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} 85.0 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 0.838 & {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 0.320 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 78.5 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 70.9 & {\cellcolor[HTML]{CBE4CB}} \color[HTML]{000000} 81.2 & {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} 77.1 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} 17.2 & {\cellcolor[HTML]{E8F2E8}} \color[HTML]{000000} 48.8 & {\cellcolor[HTML]{E8F2E8}} \color[HTML]{000000} 45.5 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 75.2 \\
ckQE(64)xcMBR & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 90.3 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 82.5 & {\cellcolor[HTML]{B1D7B1}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 1.147 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 0.720 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 71.9 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 84.1 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 77.8 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 81.5 & {\cellcolor[HTML]{C1DFC1}} \color[HTML]{000000} 18.2 & {\cellcolor[HTML]{BCDCBC}} \color[HTML]{000000} 50.1 & {\cellcolor[HTML]{BCDCBC}} \color[HTML]{000000} 46.8 & {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 73.4 \\
ckQE(32)xcMBR & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 90.1 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 1.166 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 0.729 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{81BF81}} \color[HTML]{000000} 72.2 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 77.9 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 18.5 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 50.4 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 47.1 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 73.0 \\
ckQE(16)xcMBR & {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 89.9 & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} 82.7 & {\cellcolor[HTML]{9CCD9C}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D7E9D7}} \color[HTML]{000000} 1.166 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 0.728 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 72.4 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 85.4 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 18.7 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 50.6 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 47.3 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 72.6 \\
ckQE(8)xcMBR & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 89.6 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 1.191 & {\cellcolor[HTML]{088408}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E2EFE2}} \color[HTML]{000000} 0.743 & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 72.6 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} 85.9 & {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 18.9 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 50.8 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 47.5 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 72.3 \\
ckQE(4)xcMBR & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 89.3 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 82.7 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 85.6 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 1.221 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.760 & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{63B163}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.4 & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 77.9 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 18.9 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 50.8 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 47.5 & {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 72.3 \\
mxQE(64)mxMBR & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 86.9 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.585 & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} {\cellcolor[HTML]{2D962D}} \color[HTML]{F1F1F1} 0.398 & {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{DFEDDF}} \color[HTML]{000000} 70.8 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 80.7 & {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 17.3 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 49.3 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 45.9 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 75.9 \\
mxQE(32)mxMBR & {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} 86.9 & {\cellcolor[HTML]{C0DEC0}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{CBE4CB}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{E6F1E6}} \color[HTML]{000000} {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.599 & {\cellcolor[HTML]{C9E2C8}} \color[HTML]{000000} {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 0.377 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 70.8 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 80.8 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{DEEDDE}} \color[HTML]{000000} 81.1 & {\cellcolor[HTML]{DFEDDF}} \color[HTML]{000000} 17.3 & {\cellcolor[HTML]{D7E9D7}} \color[HTML]{000000} 49.3 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 46.0 & {\cellcolor[HTML]{078407}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} 75.8 \\
mxQE(16)mxMBR & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{C8E2C8}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 0.616 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 0.356 & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 70.8 & {\cellcolor[HTML]{DEEDDE}} \color[HTML]{000000} 80.8 & {\cellcolor[HTML]{CBE4CB}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 81.1 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 17.3 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 49.2 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 45.8 & {\cellcolor[HTML]{088408}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E2EFE2}} \color[HTML]{000000} 75.8 \\
mxQE(8)mxMBR & {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 81.3 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 85.1 & {\cellcolor[HTML]{D3E7D3}} \color[HTML]{000000} {\cellcolor[HTML]{188C18}} \color[HTML]{F1F1F1} 0.651 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 0.334 & {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} 70.7 & {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 80.6 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 77.3 & {\cellcolor[HTML]{E1EEE1}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} 17.2 & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 49.0 & {\cellcolor[HTML]{E1EEE1}} \color[HTML]{000000} 45.7 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 75.9 \\
mxQE(4)mxMBR & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 86.3 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 85.0 & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} {\cellcolor[HTML]{289428}} \color[HTML]{F1F1F1} 0.695 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.311 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 70.6 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 77.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.9 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 45.4 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.2 \\
ckQE(64)mxMBR & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 87.4 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{E1EEE1}} \color[HTML]{000000} {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 0.611 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 0.433 & {\cellcolor[HTML]{C0DEC0}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 81.3 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 17.8 & {\cellcolor[HTML]{C1DFC1}} \color[HTML]{000000} 50.0 & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 46.6 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 75.1 \\
ckQE(32)mxMBR & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 87.8 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 82.5 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 0.661 & {\cellcolor[HTML]{A0CEA0}} \color[HTML]{000000} {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 0.454 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} 72.0 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 18.3 & {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 50.4 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 47.1 & {\cellcolor[HTML]{289428}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 74.2 \\
ckQE(16)mxMBR & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 88.1 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{8DC58D}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 0.723 & {\cellcolor[HTML]{91C791}} \color[HTML]{000000} {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 0.483 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 72.3 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 18.6 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 50.8 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 47.5 & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 73.5 \\
ckQE(8)mxMBR & {\cellcolor[HTML]{7ABC7A}} \color[HTML]{000000} 88.2 & {\cellcolor[HTML]{81BF81}} \color[HTML]{000000} 82.8 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{9ACB9A}} \color[HTML]{000000} {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 0.804 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 0.531 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 72.5 & {\cellcolor[HTML]{219021}} \color[HTML]{F1F1F1} 85.5 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 18.8 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} 50.9 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 47.6 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A9D3A9}} \color[HTML]{000000} 73.0 \\
ckQE(4)mxMBR & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} 88.2 & {\cellcolor[HTML]{7EBE7E}} \color[HTML]{000000} 82.9 & {\cellcolor[HTML]{8DC58D}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 0.919 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 0.594 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} 79.3 & {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{9CCD9C}} \color[HTML]{000000} 81.9 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 18.9 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} 50.9 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 47.6 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 72.7 \\
\end{tabular}


\caption{Reference-based and QE evaluation scores for greedy, MBR, and QE decoding using a two-step ensemble (QE filtering followed by MBR) utility metric, averaged across all languages (dev datasets). Higher scores are better, except MetricX, MetricX-QE, and TER, where lower is better.}
\label{tab:multistep_all_dev}
\end{small}

==> tables/singlemetric/singlemetric_all_dev.tex <==
\setlength\tabcolsep{2 pt}
\begin{small}

\begin{tabular}{lrrrrrrrrrrrrrr}
\hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \lrot{\textbf{Evaluated Metric}} & \lrot{XCOMET-XXL} & \lrot{XCOMET-XL} & \lrot{COMET22} & \lrot{MetricX} & \lrot{MetricX-QE} & \lrot{CometKiwi22} & \lrot{CometKiwi23-XL} & \lrot{CometKiwi23-XXL} & \lrot{BLEURT} & \lrot{YiSi} & \lrot{sentBLEU} & \lrot{chrF} & \lrot{chrF++} & \lrot{TER} \\
\textbf{Decoding Method} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Greedy & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 84.1 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 79.8 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 85.3 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 1.461 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 1.005 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 69.6 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 77.8 & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 24.7 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 55.6 & {\cellcolor[HTML]{219021}} \color[HTML]{F1F1F1} 52.5 & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} {\cellcolor[HTML]{389B38}} \color[HTML]{F1F1F1} 64.7 \\
XCOMET-XXL & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 88.9 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 84.9 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 1.296 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 0.837 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 70.5 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 76.9 & {\cellcolor[HTML]{D3E7D3}} \color[HTML]{000000} 81.1 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 17.2 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 49.0 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 45.7 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 75.1 \\
XCOMET-XL & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 87.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{4CA54C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 1.251 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 0.833 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 78.6 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 19.0 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 50.6 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 47.4 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 72.3 \\
COMET22 & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} 86.2 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 81.9 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 87.7 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 1.302 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} 0.869 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 71.3 & {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 83.1 & {\cellcolor[HTML]{59AC59}} \color[HTML]{F1F1F1} 22.1 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 54.0 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 50.7 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 67.7 \\
MetricX & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 81.6 & {\cellcolor[HTML]{C6E1C6}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.575 & {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 0.423 & {\cellcolor[HTML]{D6E9D6}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 70.6 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 80.5 & {\cellcolor[HTML]{C2DFC2}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{DFEDDF}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{DEEDDE}} \color[HTML]{000000} 17.0 & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 49.1 & {\cellcolor[HTML]{D1E6D1}} \color[HTML]{000000} 45.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.5 \\
MetricX-QE & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 80.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 84.7 & {\cellcolor[HTML]{ADD5AD}} \color[HTML]{000000} {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 0.839 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.274 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} 70.2 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 79.9 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.3 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.5 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 44.7 & {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} 76.2 \\
CometKiwi22 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CAE3CA}} \color[HTML]{000000} 1.439 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 0.903 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 82.4 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 71.9 & {\cellcolor[HTML]{8EC58E}} \color[HTML]{000000} 81.3 & {\cellcolor[HTML]{B7DAB7}} \color[HTML]{000000} 77.7 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 18.6 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 50.4 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 47.1 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 72.7 \\
CometKiwi23-XL & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{A9D3A9}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{399C39}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 1.335 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 0.831 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 79.4 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 76.0 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 77.7 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{B5D9B5}} \color[HTML]{000000} 18.6 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 50.6 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 47.3 & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} 73.6 \\
CometKiwi23-XXL & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 88.0 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 85.5 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 1.293 & {\cellcolor[HTML]{52A852}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{99CB99}} \color[HTML]{000000} 0.799 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 79.3 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 77.7 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 18.8 & {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 50.6 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 47.3 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 72.5 \\
BLEURT & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} 1.262 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 0.864 & {\cellcolor[HTML]{BDDCBD}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} 70.7 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} 80.1 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 82.9 & {\cellcolor[HTML]{8DC58D}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 19.8 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 51.9 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 48.5 & {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} 72.6 \\
YiSi & {\cellcolor[HTML]{D3E7D3}} \color[HTML]{000000} 84.2 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 80.0 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 1.459 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 0.994 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 70.0 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 79.0 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} 24.8 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 56.1 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} 53.1 & {\cellcolor[HTML]{C1DFC1}} \color[HTML]{000000} {\cellcolor[HTML]{299429}} \color[HTML]{F1F1F1} 63.7 \\
sentBLEU & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 83.9 & {\cellcolor[HTML]{E0EEE0}} \color[HTML]{000000} 79.8 & {\cellcolor[HTML]{B4D8B4}} \color[HTML]{000000} 85.4 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 1.501 & {\cellcolor[HTML]{0E870E}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{DDECDD}} \color[HTML]{000000} 1.030 & {\cellcolor[HTML]{E0EEDF}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{D4E8D4}} \color[HTML]{000000} 69.5 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} 78.4 & {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 77.8 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 25.6 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 55.5 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 52.7 & {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 63.3 \\
chrF & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 84.3 & {\cellcolor[HTML]{DCECDC}} \color[HTML]{000000} 79.9 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 1.425 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} 0.976 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{BDDDBD}} \color[HTML]{000000} 70.2 & {\cellcolor[HTML]{C4E0C4}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 78.4 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 83.9 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 24.5 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 57.0 & {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 53.8 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 66.1 \\
chrF++ & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 84.3 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 79.9 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 85.8 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 1.424 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} 0.978 & {\cellcolor[HTML]{D5E9D5}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{BEDDBE}} \color[HTML]{000000} 70.2 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 78.4 & {\cellcolor[HTML]{188C18}} \color[HTML]{F1F1F1} 84.0 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} 24.8 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 57.0 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 53.8 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 65.7 \\
TER & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 83.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 79.5 & {\cellcolor[HTML]{CDE5CD}} \color[HTML]{000000} 85.1 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 1.579 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 1.079 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 77.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 68.8 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 77.7 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 77.4 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 24.4 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 54.5 & {\cellcolor[HTML]{3A9C3A}} \color[HTML]{F1F1F1} 51.6 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 60.9 \\
\end{tabular}


\caption{Reference-based and QE evaluation scores for greedy, MBR, and QE decoding using a single utility metric, averaged across all languages (dev datasets). Higher scores are better, except MetricX, MetricX-QE, and TER, where lower is better. The green diagonal suggests automated metric evaluations prefer MBR outputs that were generated using the same utility metric.}
\label{tab:singlemetric_all_dev}
\end{small}

==> tables/singlemetric/singlemetric_all_test.tex <==
\makebox[\textwidth]{
\setlength\tabcolsep{2 pt}
\begin{small}

\begin{tabular}{lcccccccccccccc}
\hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \lrot{\textbf{Evaluated Metric}} & \lrot{MetricX} & \lrot{MetricX-QE} & \lrot{XCOMET-XXL} & \lrot{XCOMET-XL} & \lrot{CometKiwi23-XXL} & \lrot{CometKiwi23-XL} & \lrot{CometKiwi22} & \lrot{COMET22} & \lrot{BLEURT} & \lrot{YiSi} & \lrot{chrF} & \lrot{chrF++} & \lrot{sentBLEU} & \lrot{TER} \\
Greedy & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 1.58 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 1.16 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 82.3 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 77.8 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 76.8 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 68.2 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 77.3 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 84.3 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 57.2 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 54.2 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 26.4 & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 63.4 \\
MetricX & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 0.656‡ & {\cellcolor[HTML]{0D8A0D}} \color[HTML]{F1F1F1} \bfseries 0.557‡ & {\cellcolor[HTML]{60CE60}} \color[HTML]{000000} \bfseries 85.5‡ & {\cellcolor[HTML]{8CF18C}} \color[HTML]{000000} \bfseries 79.6‡ & {\cellcolor[HTML]{8AF08A}} \color[HTML]{000000} \bfseries 79.0‡ & {\cellcolor[HTML]{A8FCA8}} \color[HTML]{000000} \bfseries 69.4‡ & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} \bfseries 77.7‡ & {\cellcolor[HTML]{F55858}} \color[HTML]{F1F1F1} \bfseries 84.9‡ & {\cellcolor[HTML]{F64C4C}} \color[HTML]{F1F1F1} \bfseries 76.6‡ & {\cellcolor[HTML]{970000}} \color[HTML]{F1F1F1} \bfseries 81.2‡ & {\cellcolor[HTML]{BC0000}} \color[HTML]{F1F1F1} \bfseries 50.3‡ & {\cellcolor[HTML]{B80000}} \color[HTML]{F1F1F1} \bfseries 46.9‡ & {\cellcolor[HTML]{A00000}} \color[HTML]{F1F1F1} \bfseries 18.1‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 75.7‡ \\
MetricX-QE & {\cellcolor[HTML]{0F8C0F}} \color[HTML]{F1F1F1} \bfseries 0.899‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 0.349‡ & {\cellcolor[HTML]{86ED86}} \color[HTML]{000000} \bfseries 84.4‡ & {\cellcolor[HTML]{E9FEE9}} \color[HTML]{000000} \bfseries 78.2‡ & {\cellcolor[HTML]{A4FBA4}} \color[HTML]{000000} \bfseries 78.3‡ & {\cellcolor[HTML]{D1FDD1}} \color[HTML]{000000} \bfseries 68.8‡ & {\cellcolor[HTML]{F5FFF5}} \color[HTML]{000000} \bfseries 77.6‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 84.4‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 75.6‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 81.1‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 49.3‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 45.9‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 17.6‡ & {\cellcolor[HTML]{970000}} \color[HTML]{F1F1F1} \bfseries 75.3‡ \\
XCOMET-XXL & {\cellcolor[HTML]{70DB70}} \color[HTML]{000000} \bfseries 1.25‡ & {\cellcolor[HTML]{6ED96E}} \color[HTML]{000000} \bfseries 0.868‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 89.9‡ & {\cellcolor[HTML]{6ED96E}} \color[HTML]{000000} \bfseries 80.4‡ & {\cellcolor[HTML]{56C656}} \color[HTML]{000000} \bfseries 80.8‡ & {\cellcolor[HTML]{88EE88}} \color[HTML]{000000} \bfseries 69.9‡ & {\cellcolor[HTML]{B8FCB8}} \color[HTML]{000000} \bfseries 78.1‡ & {\cellcolor[HTML]{F27070}} \color[HTML]{F1F1F1} \bfseries 85.0‡ & {\cellcolor[HTML]{F64E4E}} \color[HTML]{F1F1F1} \bfseries 76.6‡ & {\cellcolor[HTML]{BF0000}} \color[HTML]{F1F1F1} \bfseries 81.5‡ & {\cellcolor[HTML]{C20000}} \color[HTML]{F1F1F1} \bfseries 50.4‡ & {\cellcolor[HTML]{BF0000}} \color[HTML]{F1F1F1} \bfseries 47.0‡ & {\cellcolor[HTML]{B20000}} \color[HTML]{F1F1F1} \bfseries 18.5‡ & {\cellcolor[HTML]{CB0000}} \color[HTML]{F1F1F1} \bfseries 73.6‡ \\
XCOMET-XL & {\cellcolor[HTML]{92F692}} \color[HTML]{000000} \bfseries 1.38‡ & {\cellcolor[HTML]{98FB98}} \color[HTML]{000000} \bfseries 1.00‡ & {\cellcolor[HTML]{45B745}} \color[HTML]{F1F1F1} \bfseries 86.4‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 85.0‡ & {\cellcolor[HTML]{66D366}} \color[HTML]{000000} \bfseries 80.2‡ & {\cellcolor[HTML]{4CBE4C}} \color[HTML]{F1F1F1} \bfseries 71.5‡ & {\cellcolor[HTML]{82E982}} \color[HTML]{000000} \bfseries 78.7‡ & {\cellcolor[HTML]{DDFEDD}} \color[HTML]{000000} \bfseries 85.3‡ & {\cellcolor[HTML]{DDFEDD}} \color[HTML]{000000} \bfseries 77.6‡ & {\cellcolor[HTML]{FE0A0A}} \color[HTML]{F1F1F1} \bfseries 82.2‡ & {\cellcolor[HTML]{FE0808}} \color[HTML]{F1F1F1} \bfseries 51.9‡ & {\cellcolor[HTML]{FE0808}} \color[HTML]{F1F1F1} \bfseries 48.7‡ & {\cellcolor[HTML]{F80000}} \color[HTML]{F1F1F1} \bfseries 20.1‡ & {\cellcolor[HTML]{FE0A0A}} \color[HTML]{F1F1F1} \bfseries 71.5‡ \\
CometKiwi23-XXL & {\cellcolor[HTML]{A8FCA8}} \color[HTML]{000000} \bfseries 1.43‡ & {\cellcolor[HTML]{86ED86}} \color[HTML]{000000} \bfseries 0.940‡ & {\cellcolor[HTML]{3DB13D}} \color[HTML]{F1F1F1} \bfseries 86.6‡ & {\cellcolor[HTML]{70DB70}} \color[HTML]{000000} \bfseries 80.4‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 85.5‡ & {\cellcolor[HTML]{4EC04E}} \color[HTML]{F1F1F1} \bfseries 71.4‡ & {\cellcolor[HTML]{84EB84}} \color[HTML]{000000} \bfseries 78.7‡ & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{F55454}} \color[HTML]{F1F1F1} \bfseries 76.7‡ & {\cellcolor[HTML]{FE0A0A}} \color[HTML]{F1F1F1} \bfseries 82.2‡ & {\cellcolor[HTML]{FE0000}} \color[HTML]{F1F1F1} \bfseries 51.7‡ & {\cellcolor[HTML]{FE0000}} \color[HTML]{F1F1F1} \bfseries 48.4‡ & {\cellcolor[HTML]{F20000}} \color[HTML]{F1F1F1} \bfseries 19.9‡ & {\cellcolor[HTML]{FE0606}} \color[HTML]{F1F1F1} \bfseries 71.7‡ \\
CometKiwi23-XL & {\cellcolor[HTML]{BCFCBC}} \color[HTML]{000000} \bfseries 1.46‡ & {\cellcolor[HTML]{92F692}} \color[HTML]{000000} \bfseries 0.978‡ & {\cellcolor[HTML]{70DB70}} \color[HTML]{000000} \bfseries 85.0‡ & {\cellcolor[HTML]{4BBC4B}} \color[HTML]{F1F1F1} \bfseries 81.5‡ & {\cellcolor[HTML]{47B947}} \color[HTML]{F1F1F1} \bfseries 81.3‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 74.8‡ & {\cellcolor[HTML]{7CE47C}} \color[HTML]{000000} \bfseries 78.8‡ & {\cellcolor[HTML]{FDFFFD}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{F46262}} \color[HTML]{F1F1F1} \bfseries 76.8‡ & {\cellcolor[HTML]{FF0404}} \color[HTML]{F1F1F1} \bfseries 82.1‡ & {\cellcolor[HTML]{FE0000}} \color[HTML]{F1F1F1} \bfseries 51.7‡ & {\cellcolor[HTML]{FE0000}} \color[HTML]{F1F1F1} \bfseries 48.4‡ & {\cellcolor[HTML]{EC0000}} \color[HTML]{F1F1F1} \bfseries 19.8‡ & {\cellcolor[HTML]{EC0000}} \color[HTML]{F1F1F1} \bfseries 72.6‡ \\
CometKiwi22 & {\cellcolor[HTML]{F9FFF9}} \color[HTML]{000000} \bfseries 1.57‡ & {\cellcolor[HTML]{C4FDC4}} \color[HTML]{000000} \bfseries 1.07‡ & {\cellcolor[HTML]{94F894}} \color[HTML]{000000} \bfseries 84.0‡ & {\cellcolor[HTML]{8CF18C}} \color[HTML]{000000} \bfseries 79.6‡ & {\cellcolor[HTML]{74DE74}} \color[HTML]{000000} \bfseries 79.7‡ & {\cellcolor[HTML]{72DC72}} \color[HTML]{000000} \bfseries 70.5‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 81.9‡ & {\cellcolor[HTML]{D1FDD1}} \color[HTML]{000000} \bfseries 85.4‡ & {\cellcolor[HTML]{F26C6C}} \color[HTML]{F1F1F1} \bfseries 76.8‡ & {\cellcolor[HTML]{FD1212}} \color[HTML]{F1F1F1} \bfseries 82.3‡ & {\cellcolor[HTML]{FE0606}} \color[HTML]{F1F1F1} \bfseries 51.9‡ & {\cellcolor[HTML]{FF0404}} \color[HTML]{F1F1F1} \bfseries 48.6‡ & {\cellcolor[HTML]{F80000}} \color[HTML]{F1F1F1} \bfseries 20.1‡ & {\cellcolor[HTML]{FD1414}} \color[HTML]{F1F1F1} \bfseries 71.0‡ \\
COMET22 & {\cellcolor[HTML]{98FB98}} \color[HTML]{000000} \bfseries 1.40‡ & {\cellcolor[HTML]{A4FBA4}} \color[HTML]{000000} \bfseries 1.02‡ & {\cellcolor[HTML]{7AE37A}} \color[HTML]{000000} \bfseries 84.7‡ & {\cellcolor[HTML]{7EE67E}} \color[HTML]{000000} \bfseries 80.0‡ & {\cellcolor[HTML]{82E982}} \color[HTML]{000000} \bfseries 79.3‡ & {\cellcolor[HTML]{84EB84}} \color[HTML]{000000} \bfseries 70.0‡ & {\cellcolor[HTML]{84EB84}} \color[HTML]{000000} \bfseries 78.7‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 87.4‡ & {\cellcolor[HTML]{B0FCB0}} \color[HTML]{000000} \bfseries 78.1‡ & {\cellcolor[HTML]{F17474}} \color[HTML]{F1F1F1} \bfseries 83.5‡ & {\cellcolor[HTML]{F17474}} \color[HTML]{F1F1F1} \bfseries 55.3‡ & {\cellcolor[HTML]{F27070}} \color[HTML]{F1F1F1} \bfseries 52.0‡ & {\cellcolor[HTML]{F55656}} \color[HTML]{F1F1F1} \bfseries 23.2‡ & {\cellcolor[HTML]{F36868}} \color[HTML]{F1F1F1} \bfseries 67.0‡ \\
BLEURT & {\cellcolor[HTML]{8CF18C}} \color[HTML]{000000} \bfseries 1.35‡ & {\cellcolor[HTML]{94F894}} \color[HTML]{000000} \bfseries 0.986‡ & {\cellcolor[HTML]{9CFB9C}} \color[HTML]{000000} \bfseries 83.8‡ & {\cellcolor[HTML]{A0FBA0}} \color[HTML]{000000} \bfseries 79.1‡ & {\cellcolor[HTML]{96F996}} \color[HTML]{000000} \bfseries 78.6‡ & {\cellcolor[HTML]{A4FBA4}} \color[HTML]{000000} \bfseries 69.4‡ & {\cellcolor[HTML]{B8FCB8}} \color[HTML]{000000} \bfseries 78.1‡ & {\cellcolor[HTML]{BCFCBC}} \color[HTML]{000000} \bfseries 85.5‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 82.3‡ & {\cellcolor[HTML]{FA2C2C}} \color[HTML]{F1F1F1} \bfseries 82.6‡ & {\cellcolor[HTML]{F93232}} \color[HTML]{F1F1F1} \bfseries 53.2‡ & {\cellcolor[HTML]{FA2C2C}} \color[HTML]{F1F1F1} \bfseries 49.8‡ & {\cellcolor[HTML]{FC1616}} \color[HTML]{F1F1F1} \bfseries 21.0‡ & {\cellcolor[HTML]{FD0E0E}} \color[HTML]{F1F1F1} \bfseries 71.3‡ \\
YiSi & {\cellcolor[HTML]{F9FFF9}} \color[HTML]{000000} 1.57 & {\cellcolor[HTML]{F1FEF1}} \color[HTML]{000000} \bfseries 1.14† & {\cellcolor[HTML]{F1FEF1}} \color[HTML]{000000} \bfseries 82.6‡ & {\cellcolor[HTML]{F5FFF5}} \color[HTML]{000000} \bfseries 78.0* & {\cellcolor[HTML]{DDFEDD}} \color[HTML]{000000} \bfseries 77.3‡ & {\cellcolor[HTML]{DDFEDD}} \color[HTML]{000000} \bfseries 68.7‡ & {\cellcolor[HTML]{E5FEE5}} \color[HTML]{000000} \bfseries 77.7‡ & {\cellcolor[HTML]{9CFB9C}} \color[HTML]{000000} \bfseries 85.6‡ & {\cellcolor[HTML]{D5FDD5}} \color[HTML]{000000} \bfseries 77.7‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 85.0‡ & {\cellcolor[HTML]{72DC72}} \color[HTML]{000000} \bfseries 57.7‡ & {\cellcolor[HTML]{7AE37A}} \color[HTML]{000000} \bfseries 54.5‡ & {\cellcolor[HTML]{FCE9E9}} \color[HTML]{000000} \bfseries 26.1* & {\cellcolor[HTML]{98FB98}} \color[HTML]{000000} 62.6 \\
chrF & {\cellcolor[HTML]{E5FEE5}} \color[HTML]{000000} \bfseries 1.54‡ & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} \bfseries 1.13† & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} \bfseries 82.6‡ & {\cellcolor[HTML]{F5FFF5}} \color[HTML]{000000} \bfseries 78.0* & {\cellcolor[HTML]{D1FDD1}} \color[HTML]{000000} \bfseries 77.6‡ & {\cellcolor[HTML]{C8FDC8}} \color[HTML]{000000} \bfseries 68.9‡ & {\cellcolor[HTML]{E5FEE5}} \color[HTML]{000000} \bfseries 77.7‡ & {\cellcolor[HTML]{94F894}} \color[HTML]{000000} \bfseries 85.7‡ & {\cellcolor[HTML]{CDFDCD}} \color[HTML]{000000} \bfseries 77.8‡ & {\cellcolor[HTML]{70DB70}} \color[HTML]{000000} \bfseries 84.5‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 58.6‡ & {\cellcolor[HTML]{006D00}} \color[HTML]{F1F1F1} \bfseries 55.3‡ & {\cellcolor[HTML]{FAD5D5}} \color[HTML]{000000} \bfseries 25.8‡ & {\cellcolor[HTML]{F5A8A8}} \color[HTML]{000000} \bfseries 65.1‡ \\
chrF++ & {\cellcolor[HTML]{E5FEE5}} \color[HTML]{000000} \bfseries 1.54‡ & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} \bfseries 1.13† & {\cellcolor[HTML]{EDFEED}} \color[HTML]{000000} \bfseries 82.6‡ & {\cellcolor[HTML]{F1FEF1}} \color[HTML]{000000} \bfseries 78.0† & {\cellcolor[HTML]{D5FDD5}} \color[HTML]{000000} \bfseries 77.5‡ & {\cellcolor[HTML]{CDFDCD}} \color[HTML]{000000} \bfseries 68.9‡ & {\cellcolor[HTML]{E5FEE5}} \color[HTML]{000000} \bfseries 77.7‡ & {\cellcolor[HTML]{96F996}} \color[HTML]{000000} \bfseries 85.6‡ & {\cellcolor[HTML]{C4FDC4}} \color[HTML]{000000} \bfseries 77.9‡ & {\cellcolor[HTML]{5ECC5E}} \color[HTML]{000000} \bfseries 84.6‡ & {\cellcolor[HTML]{006D00}} \color[HTML]{F1F1F1} \bfseries 58.6‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 55.4‡ & {\cellcolor[HTML]{FEF3F3}} \color[HTML]{000000} 26.2 & {\cellcolor[HTML]{F8C1C1}} \color[HTML]{000000} \bfseries 64.6† \\
sentBLEU & {\cellcolor[HTML]{F49E9E}} \color[HTML]{000000} 1.61 & {\cellcolor[HTML]{F18A8A}} \color[HTML]{F1F1F1} \bfseries 1.18* & {\cellcolor[HTML]{F36666}} \color[HTML]{F1F1F1} \bfseries 82.2* & {\cellcolor[HTML]{F5ADAD}} \color[HTML]{000000} \bfseries 77.8* & {\cellcolor[HTML]{FEF8F8}} \color[HTML]{000000} 76.8 & {\cellcolor[HTML]{FBDFDF}} \color[HTML]{000000} 68.2 & {\cellcolor[HTML]{FBDFDF}} \color[HTML]{000000} 77.5 & {\cellcolor[HTML]{F1FEF1}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{FEF3F3}} \color[HTML]{000000} \bfseries 77.3* & {\cellcolor[HTML]{E1FEE1}} \color[HTML]{000000} 84.3 & {\cellcolor[HTML]{FDEEEE}} \color[HTML]{000000} \bfseries 57.0‡ & {\cellcolor[HTML]{FFFDFD}} \color[HTML]{000000} \bfseries 54.1* & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 27.1‡ & {\cellcolor[HTML]{82E982}} \color[HTML]{000000} 62.3 \\
TER & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 1.74‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 1.27‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 81.9‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 77.2‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 75.9‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 67.5‡ & {\cellcolor[HTML]{8B0000}} \color[HTML]{F1F1F1} \bfseries 77.2‡ & {\cellcolor[HTML]{FC1C1C}} \color[HTML]{F1F1F1} \bfseries 84.7‡ & {\cellcolor[HTML]{F55454}} \color[HTML]{F1F1F1} \bfseries 76.7‡ & {\cellcolor[HTML]{F5ADAD}} \color[HTML]{000000} \bfseries 83.9‡ & {\cellcolor[HTML]{F08080}} \color[HTML]{F1F1F1} \bfseries 55.7‡ & {\cellcolor[HTML]{F28F8F}} \color[HTML]{F1F1F1} \bfseries 52.7‡ & {\cellcolor[HTML]{F8C6C6}} \color[HTML]{000000} \bfseries 25.6‡ & {\cellcolor[HTML]{006400}} \color[HTML]{F1F1F1} \bfseries 59.7‡ \\
\end{tabular}


\end{small}
}
\begin{small}
  

\caption{Reference-based and QE evaluation scores for greedy, MBR, and QE decoding using a single utility metric, averaged across all languages (test datasets). Higher scores are better, except MetricX, MetricX-QE, and TER, where lower is better. The green diagonal suggests automated metric evaluations prefer MBR outputs that were generated using the same utility metric. Significant differences from greedy (pairwise t-test) indicated by * for p<0.05, † for p<0.01, ‡ for p<0.001.}
\label{tab:singlemetric_all_test}
\end{small}

==> tables/singlestep/singlestep_all_dev.tex <==
\setlength\tabcolsep{2 pt}
\begin{small}

\begin{tabular}{lrrrrrrrrrrrrrr}
\hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \hfill \lrot{\textbf{Evaluated Metric}} & \lrot{XCOMET-XXL} & \lrot{XCOMET-XL} & \lrot{COMET22} & \lrot{MetricX} & \lrot{MetricX-QE} & \lrot{CometKiwi22} & \lrot{CometKiwi23-XL} & \lrot{CometKiwi23-XXL} & \lrot{BLEURT} & \lrot{YiSi} & \lrot{sentBLEU} & \lrot{chrF} & \lrot{chrF++} & \lrot{TER} \\
\textbf{Decoding Method} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
rankAvg:all & {\cellcolor[HTML]{58AB58}} \color[HTML]{F1F1F1} 87.8 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 0.973 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 0.606 & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 79.7 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 72.6 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{0F870F}} \color[HTML]{F1F1F1} 83.8 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 24.0 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 55.7 & {\cellcolor[HTML]{118911}} \color[HTML]{F1F1F1} 52.5 & {\cellcolor[HTML]{D8EAD8}} \color[HTML]{000000} {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 64.7 \\
rankAvg:qe & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 88.0 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 86.2 & {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.948 & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.477 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 80.8 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} 74.2 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 78.6 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 19.5 & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} 51.7 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 48.4 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 71.9 \\
rankAvg:top & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 89.1 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 84.7 & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} 0.814 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 0.457 & {\cellcolor[HTML]{73B873}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{209020}} \color[HTML]{F1F1F1} 74.0 & {\cellcolor[HTML]{309730}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{4EA64E}} \color[HTML]{F1F1F1} 79.1 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 19.5 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 51.7 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 48.4 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 71.9 \\
rankAvg:topQe & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 88.0 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 85.9 & {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 0.919 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 0.435 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 74.6 & {\cellcolor[HTML]{0E870E}} \color[HTML]{F1F1F1} 85.3 & {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 81.9 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 19.1 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 51.1 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 47.8 & {\cellcolor[HTML]{45A245}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 72.7 \\
rankAvg:mxmxqe & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 87.0 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{B9DBB9}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.610 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.315 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 71.0 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 77.6 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 17.2 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 49.2 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 45.8 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 76.1 \\
rankAvg:noLex & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 88.5 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 84.1 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 0.888 & {\cellcolor[HTML]{7CBD7C}} \color[HTML]{000000} {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} 0.532 & {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 80.1 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 73.3 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 80.4 & {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 22.3 & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} 54.4 & {\cellcolor[HTML]{3A9C3A}} \color[HTML]{F1F1F1} 51.1 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 67.6 \\
rankAvg:noNC & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 86.7 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 82.3 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{4DA64D}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9DCD9D}} \color[HTML]{000000} 0.993 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 0.608 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{B6D9B6}} \color[HTML]{000000} 71.3 & {\cellcolor[HTML]{BFDEBF}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{078407}} \color[HTML]{F1F1F1} 83.9 & {\cellcolor[HTML]{0C860C}} \color[HTML]{F1F1F1} 24.4 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 56.0 & {\cellcolor[HTML]{0A850A}} \color[HTML]{F1F1F1} 52.8 & {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 63.9 \\
rankAvg:noNCnoLex & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} 87.2 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 82.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 0.876 & {\cellcolor[HTML]{84C084}} \color[HTML]{000000} {\cellcolor[HTML]{67B267}} \color[HTML]{F1F1F1} 0.518 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{9CCD9C}} \color[HTML]{000000} 71.8 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 80.4 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 22.7 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 54.8 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 51.5 & {\cellcolor[HTML]{B0D6B0}} \color[HTML]{000000} {\cellcolor[HTML]{3B9D3B}} \color[HTML]{F1F1F1} 66.9 \\
rankAvg:noNCQe & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.3 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 0.877 & {\cellcolor[HTML]{E8F2E8}} \color[HTML]{000000} {\cellcolor[HTML]{038103}} \color[HTML]{F1F1F1} 0.321 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 70.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.5 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 44.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.5 \\
rankMax:all & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 87.4 & {\cellcolor[HTML]{64B164}} \color[HTML]{F1F1F1} 82.9 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B8DAB8}} \color[HTML]{000000} 1.058 & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 0.642 & {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 79.7 & {\cellcolor[HTML]{7ABC7A}} \color[HTML]{000000} 72.4 & {\cellcolor[HTML]{86C286}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 23.1 & {\cellcolor[HTML]{2C962C}} \color[HTML]{F1F1F1} 54.8 & {\cellcolor[HTML]{2E972E}} \color[HTML]{F1F1F1} 51.6 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 65.3 \\
rankMax:qe & {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} 87.7 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 86.2 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 0.977 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 0.493 & {\cellcolor[HTML]{0B850B}} \color[HTML]{F1F1F1} 80.7 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 73.9 & {\cellcolor[HTML]{339933}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 78.6 & {\cellcolor[HTML]{81BF81}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 19.7 & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 51.8 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} 48.5 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 71.5 \\
rankMax:top & {\cellcolor[HTML]{0E870E}} \color[HTML]{F1F1F1} 88.9 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{65B265}} \color[HTML]{F1F1F1} 86.0 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 0.849 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} 0.480 & {\cellcolor[HTML]{85C185}} \color[HTML]{000000} 79.3 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 72.6 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 84.2 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 78.9 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 19.5 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 51.6 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 48.3 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 71.6 \\
rankMax:topQe & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 88.1 & {\cellcolor[HTML]{72B872}} \color[HTML]{F1F1F1} 82.6 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.885 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 0.390 & {\cellcolor[HTML]{90C790}} \color[HTML]{000000} 79.2 & {\cellcolor[HTML]{70B770}} \color[HTML]{F1F1F1} 72.5 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 85.6 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 18.5 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 50.5 & {\cellcolor[HTML]{A8D2A8}} \color[HTML]{000000} 47.2 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{AAD3AA}} \color[HTML]{000000} 73.0 \\
rankMax:mxmxqe & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 86.9 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 0.612 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 0.317 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{CAE3CA}} \color[HTML]{000000} 70.9 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 77.6 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 17.1 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 49.2 & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 45.8 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 76.1 \\
rankMax:noLex & {\cellcolor[HTML]{5FAE5F}} \color[HTML]{F1F1F1} 87.7 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 83.2 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 1.010 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 0.610 & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 72.7 & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{219021}} \color[HTML]{F1F1F1} 79.8 & {\cellcolor[HTML]{2F972F}} \color[HTML]{F1F1F1} 83.4 & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 22.2 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 54.2 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 51.0 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} 67.5 \\
rankMax:noNC & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{8CC58C}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{229122}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 1.010 & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 0.598 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{BBDCBB}} \color[HTML]{000000} 71.2 & {\cellcolor[HTML]{C1DFC1}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 23.5 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} 55.0 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 51.9 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 64.6 \\
rankMax:noNCnoLex & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 86.8 & {\cellcolor[HTML]{7EBE7E}} \color[HTML]{000000} 82.4 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 0.948 & {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} 0.555 & {\cellcolor[HTML]{9CCD9C}} \color[HTML]{000000} 79.0 & {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 71.5 & {\cellcolor[HTML]{B2D7B2}} \color[HTML]{000000} 81.4 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 80.2 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{40A040}} \color[HTML]{F1F1F1} 22.6 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 54.6 & {\cellcolor[HTML]{349934}} \color[HTML]{F1F1F1} 51.3 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 67.0 \\
rankMax:noNCQe & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.3 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.881 & {\cellcolor[HTML]{E6F1E6}} \color[HTML]{000000} {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 0.325 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 70.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.8 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.6 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 44.8 & {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 76.4 \\
rankMed:all & {\cellcolor[HTML]{5BAD5B}} \color[HTML]{F1F1F1} 87.8 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 0.974 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 0.614 & {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 72.5 & {\cellcolor[HTML]{80BF80}} \color[HTML]{000000} 82.6 & {\cellcolor[HTML]{1A8D1A}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{1F8F1F}} \color[HTML]{F1F1F1} 23.7 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 55.4 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 52.3 & {\cellcolor[HTML]{C8E2C8}} \color[HTML]{000000} {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 65.6 \\
rankMed:qe & {\cellcolor[HTML]{57AB57}} \color[HTML]{F1F1F1} 87.8 & {\cellcolor[HTML]{42A042}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{66B266}} \color[HTML]{F1F1F1} 86.0 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{ADD5AD}} \color[HTML]{000000} 1.031 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} 0.557 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 80.5 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 74.2 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 84.9 & {\cellcolor[HTML]{78BB78}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 19.0 & {\cellcolor[HTML]{96C996}} \color[HTML]{000000} 51.1 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 47.8 & {\cellcolor[HTML]{46A246}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 72.7 \\
rankMed:top & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 89.1 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 84.8 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 85.9 & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 0.821 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 0.470 & {\cellcolor[HTML]{76BA76}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{2A952A}} \color[HTML]{F1F1F1} 73.8 & {\cellcolor[HTML]{369B36}} \color[HTML]{F1F1F1} 84.3 & {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} 78.7 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 18.8 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 51.0 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 47.7 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{ACD4AC}} \color[HTML]{000000} 73.1 \\
rankMed:topQe & {\cellcolor[HTML]{55A955}} \color[HTML]{F1F1F1} 87.9 & {\cellcolor[HTML]{4CA54C}} \color[HTML]{F1F1F1} 83.3 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{249224}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{C7E1C7}} \color[HTML]{000000} 1.093 & {\cellcolor[HTML]{5CAD5C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} 0.596 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 74.4 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 85.2 & {\cellcolor[HTML]{8DC58D}} \color[HTML]{000000} 78.0 & {\cellcolor[HTML]{A6D1A6}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{B2D7B1}} \color[HTML]{000000} 18.6 & {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 50.5 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 47.2 & {\cellcolor[HTML]{379B37}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{B3D8B3}} \color[HTML]{000000} 73.5 \\
rankMed:mxmxqe & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 87.0 & {\cellcolor[HTML]{9ECE9E}} \color[HTML]{000000} 81.8 & {\cellcolor[HTML]{B9DBB9}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.610 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.315 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 71.0 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{A3D0A3}} \color[HTML]{000000} 77.6 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{D9EAD9}} \color[HTML]{000000} 17.2 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 49.2 & {\cellcolor[HTML]{CFE5CF}} \color[HTML]{000000} 45.8 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E4F0E4}} \color[HTML]{000000} 76.1 \\
rankMed:noLex & {\cellcolor[HTML]{1B8D1B}} \color[HTML]{F1F1F1} 88.7 & {\cellcolor[HTML]{108810}} \color[HTML]{F1F1F1} 84.5 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{8AC48A}} \color[HTML]{000000} {\cellcolor[HTML]{61AF61}} \color[HTML]{F1F1F1} 0.846 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} {\cellcolor[HTML]{61B061}} \color[HTML]{F1F1F1} 0.507 & {\cellcolor[HTML]{4BA54B}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 73.4 & {\cellcolor[HTML]{4FA74F}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{5AAC5A}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 21.0 & {\cellcolor[HTML]{5CAD5C}} \color[HTML]{F1F1F1} 53.1 & {\cellcolor[HTML]{5EAE5E}} \color[HTML]{F1F1F1} 49.8 & {\cellcolor[HTML]{7ABC7A}} \color[HTML]{000000} {\cellcolor[HTML]{70B770}} \color[HTML]{F1F1F1} 69.8 \\
rankMed:noNC & {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{ABD4AB}} \color[HTML]{000000} 81.5 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 86.3 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 1.181 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 0.776 & {\cellcolor[HTML]{BDDCBD}} \color[HTML]{000000} 78.7 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} 70.8 & {\cellcolor[HTML]{E2EFE2}} \color[HTML]{000000} 80.2 & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} 79.2 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 84.0 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 24.9 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 56.3 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 53.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 63.7 \\
rankMed:noNCnoLex & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 87.2 & {\cellcolor[HTML]{6DB56D}} \color[HTML]{F1F1F1} 82.7 & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{8DC58D}} \color[HTML]{000000} {\cellcolor[HTML]{5EAE5E}} \color[HTML]{F1F1F1} 0.839 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} 0.504 & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{9FCE9F}} \color[HTML]{000000} 71.7 & {\cellcolor[HTML]{A5D1A5}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 83.0 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 21.8 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 53.8 & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 50.5 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} {\cellcolor[HTML]{60AF60}} \color[HTML]{F1F1F1} 68.9 \\
rankMed:noNCQe & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.3 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 0.877 & {\cellcolor[HTML]{E8F2E8}} \color[HTML]{000000} {\cellcolor[HTML]{038103}} \color[HTML]{F1F1F1} 0.321 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 78.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 70.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.5 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 44.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.5 \\
rank75q:all & {\cellcolor[HTML]{5DAE5D}} \color[HTML]{F1F1F1} 87.8 & {\cellcolor[HTML]{43A143}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{128912}} \color[HTML]{F1F1F1} 86.7 & {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 0.986 & {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} 0.613 & {\cellcolor[HTML]{6AB46A}} \color[HTML]{F1F1F1} 79.6 & {\cellcolor[HTML]{6EB66E}} \color[HTML]{F1F1F1} 72.6 & {\cellcolor[HTML]{7ABC7A}} \color[HTML]{000000} 82.7 & {\cellcolor[HTML]{1C8E1C}} \color[HTML]{F1F1F1} 79.9 & {\cellcolor[HTML]{138913}} \color[HTML]{F1F1F1} 83.7 & {\cellcolor[HTML]{1D8E1D}} \color[HTML]{F1F1F1} 23.8 & {\cellcolor[HTML]{158A15}} \color[HTML]{F1F1F1} 55.6 & {\cellcolor[HTML]{168B16}} \color[HTML]{F1F1F1} 52.4 & {\cellcolor[HTML]{D2E7D2}} \color[HTML]{000000} {\cellcolor[HTML]{198C19}} \color[HTML]{F1F1F1} 65.1 \\
rank75q:qe & {\cellcolor[HTML]{51A851}} \color[HTML]{F1F1F1} 87.9 & {\cellcolor[HTML]{3E9E3E}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 0.973 & {\cellcolor[HTML]{8FC68F}} \color[HTML]{000000} {\cellcolor[HTML]{5CAD5C}} \color[HTML]{F1F1F1} 0.497 & {\cellcolor[HTML]{178B17}} \color[HTML]{F1F1F1} 80.5 & {\cellcolor[HTML]{148A14}} \color[HTML]{F1F1F1} 74.2 & {\cellcolor[HTML]{239123}} \color[HTML]{F1F1F1} 84.7 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 78.6 & {\cellcolor[HTML]{84C184}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 19.5 & {\cellcolor[HTML]{87C287}} \color[HTML]{000000} 51.6 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} 48.3 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{97CA97}} \color[HTML]{000000} 71.9 \\
rank75q:top & {\cellcolor[HTML]{038103}} \color[HTML]{F1F1F1} 89.1 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 84.7 & {\cellcolor[HTML]{5EAE5E}} \color[HTML]{F1F1F1} 86.1 & {\cellcolor[HTML]{98CA98}} \color[HTML]{000000} {\cellcolor[HTML]{53A953}} \color[HTML]{F1F1F1} 0.811 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} {\cellcolor[HTML]{49A449}} \color[HTML]{F1F1F1} 0.459 & {\cellcolor[HTML]{77BA77}} \color[HTML]{F1F1F1} 79.5 & {\cellcolor[HTML]{269226}} \color[HTML]{F1F1F1} 73.9 & {\cellcolor[HTML]{349934}} \color[HTML]{F1F1F1} 84.4 & {\cellcolor[HTML]{54A954}} \color[HTML]{F1F1F1} 79.0 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 82.1 & {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 19.4 & {\cellcolor[HTML]{8BC48B}} \color[HTML]{000000} 51.5 & {\cellcolor[HTML]{8CC58C}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{50A750}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{9BCC9B}} \color[HTML]{000000} 72.1 \\
rank75q:topQe & {\cellcolor[HTML]{4BA54A}} \color[HTML]{F1F1F1} 88.0 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 83.6 & {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 85.9 & {\cellcolor[HTML]{6CB56C}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{7FBE7F}} \color[HTML]{000000} 0.918 & {\cellcolor[HTML]{AED5AE}} \color[HTML]{000000} {\cellcolor[HTML]{3D9E3D}} \color[HTML]{F1F1F1} 0.435 & {\cellcolor[HTML]{78BB78}} \color[HTML]{F1F1F1} 79.4 & {\cellcolor[HTML]{028102}} \color[HTML]{F1F1F1} 74.5 & {\cellcolor[HTML]{118811}} \color[HTML]{F1F1F1} 85.2 & {\cellcolor[HTML]{75B975}} \color[HTML]{F1F1F1} 78.4 & {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 82.0 & {\cellcolor[HTML]{A2CFA2}} \color[HTML]{000000} 19.1 & {\cellcolor[HTML]{93C893}} \color[HTML]{000000} 51.2 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} 47.9 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 72.6 \\
rank75q:mxmxqe & {\cellcolor[HTML]{94C994}} \color[HTML]{000000} 86.9 & {\cellcolor[HTML]{A0CEA0}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 85.2 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} {\cellcolor[HTML]{018001}} \color[HTML]{F1F1F1} 0.612 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} 0.316 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 78.3 & {\cellcolor[HTML]{C9E3C9}} \color[HTML]{000000} 70.9 & {\cellcolor[HTML]{C5E0C5}} \color[HTML]{000000} 80.9 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 77.6 & {\cellcolor[HTML]{DBEBDB}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{DAEBDA}} \color[HTML]{000000} 17.1 & {\cellcolor[HTML]{CEE5CE}} \color[HTML]{000000} 49.2 & {\cellcolor[HTML]{D0E6D0}} \color[HTML]{000000} 45.8 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{E5F0E5}} \color[HTML]{000000} 76.1 \\
rank75q:noLex & {\cellcolor[HTML]{2B952B}} \color[HTML]{F1F1F1} 88.5 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 84.2 & {\cellcolor[HTML]{088408}} \color[HTML]{F1F1F1} 86.8 & {\cellcolor[HTML]{79BC79}} \color[HTML]{000000} {\cellcolor[HTML]{71B771}} \color[HTML]{F1F1F1} 0.885 & {\cellcolor[HTML]{7DBD7D}} \color[HTML]{000000} {\cellcolor[HTML]{6DB66D}} \color[HTML]{F1F1F1} 0.531 & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} 80.0 & {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 73.2 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 83.5 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 80.3 & {\cellcolor[HTML]{3F9F3F}} \color[HTML]{F1F1F1} 83.1 & {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 21.8 & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} 53.9 & {\cellcolor[HTML]{47A347}} \color[HTML]{F1F1F1} 50.7 & {\cellcolor[HTML]{95C995}} \color[HTML]{000000} {\cellcolor[HTML]{56AA56}} \color[HTML]{F1F1F1} 68.4 \\
rank75q:noNC & {\cellcolor[HTML]{AFD6AF}} \color[HTML]{000000} 86.5 & {\cellcolor[HTML]{89C389}} \color[HTML]{000000} 82.2 & {\cellcolor[HTML]{1E8F1E}} \color[HTML]{F1F1F1} 86.6 & {\cellcolor[HTML]{41A041}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A9D3A9}} \color[HTML]{000000} 1.022 & {\cellcolor[HTML]{44A144}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{A6D2A6}} \color[HTML]{000000} 0.642 & {\cellcolor[HTML]{A7D2A7}} \color[HTML]{000000} 78.9 & {\cellcolor[HTML]{BADBBA}} \color[HTML]{000000} 71.2 & {\cellcolor[HTML]{C3E0C3}} \color[HTML]{000000} 81.0 & {\cellcolor[HTML]{279327}} \color[HTML]{F1F1F1} 79.7 & {\cellcolor[HTML]{098509}} \color[HTML]{F1F1F1} 83.9 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 24.4 & {\cellcolor[HTML]{0C860C}} \color[HTML]{F1F1F1} 55.9 & {\cellcolor[HTML]{0D860D}} \color[HTML]{F1F1F1} 52.7 & {\cellcolor[HTML]{E3EFE3}} \color[HTML]{000000} {\cellcolor[HTML]{078407}} \color[HTML]{F1F1F1} 64.1 \\
rank75q:noNCnoLex & {\cellcolor[HTML]{82C082}} \color[HTML]{000000} 87.2 & {\cellcolor[HTML]{6BB46B}} \color[HTML]{F1F1F1} 82.8 & {\cellcolor[HTML]{058205}} \color[HTML]{F1F1F1} 86.9 & {\cellcolor[HTML]{83C083}} \color[HTML]{000000} {\cellcolor[HTML]{68B368}} \color[HTML]{F1F1F1} 0.863 & {\cellcolor[HTML]{88C388}} \color[HTML]{000000} {\cellcolor[HTML]{62B062}} \color[HTML]{F1F1F1} 0.510 & {\cellcolor[HTML]{92C892}} \color[HTML]{000000} 79.1 & {\cellcolor[HTML]{9CCD9C}} \color[HTML]{000000} 71.8 & {\cellcolor[HTML]{A4D0A4}} \color[HTML]{000000} 81.7 & {\cellcolor[HTML]{068306}} \color[HTML]{F1F1F1} 80.3 & {\cellcolor[HTML]{329832}} \color[HTML]{F1F1F1} 83.3 & {\cellcolor[HTML]{48A348}} \color[HTML]{F1F1F1} 22.3 & {\cellcolor[HTML]{3A9C3A}} \color[HTML]{F1F1F1} 54.3 & {\cellcolor[HTML]{3C9D3C}} \color[HTML]{F1F1F1} 51.0 & {\cellcolor[HTML]{A1CFA1}} \color[HTML]{000000} {\cellcolor[HTML]{4AA44A}} \color[HTML]{F1F1F1} 67.7 \\
rank75q:noNCQe & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 85.7 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.3 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 84.8 & {\cellcolor[HTML]{7BBC7B}} \color[HTML]{000000} {\cellcolor[HTML]{6FB76F}} \color[HTML]{F1F1F1} 0.881 & {\cellcolor[HTML]{E7F1E7}} \color[HTML]{000000} {\cellcolor[HTML]{048204}} \color[HTML]{F1F1F1} 0.323 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 78.1 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 70.4 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 80.0 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.4 & {\cellcolor[HTML]{EAF2EA}} \color[HTML]{000000} 80.8 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 16.6 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 44.8 & {\cellcolor[HTML]{008000}} \color[HTML]{F1F1F1} {\cellcolor[HTML]{EBF3EB}} \color[HTML]{000000} 76.4 \\
\end{tabular}


\caption{Reference-based and QE evaluation scores for greedy, MBR, and QE decoding using a single-step ensemble utility metric, averaged across all languages (dev datasets). Higher scores are better, except MetricX, MetricX-QE, and TER, where lower is better.}
\label{tab:singlestep_all_dev}
\end{small}
